Geographical Load Balancing across Green Datacenters

"Geographic Load Balancing" is a strategy for reducing the energy cost of data centers spreading across different terrestrial locations. In this paper, we focus on load balancing among micro-datacenters powered by renewable energy sources. We model via a Markov Chain the problem of scheduling jobs by prioritizing datacenters where renewable energy is currently available. Not finding a convenient closed form solution for the resulting chain, we use mean field techniques to derive an asymptotic approximate model which instead is shown to have an extremely simple and intuitive steady state solution. After proving, using both theoretical and discrete event simulation results, that the system performance converges to the asymptotic model for an increasing number of datacenters, we exploit the simple closed form model's solution to investigate relationships and trade-offs among the various system parameters.

==> RELATED.tex <==
%!TEX root = papero.tex

\section{Related Work\label{RELATED}}
In Geographic Load Balancing (GLB) systems user requests are initially accepted
by front-end elements and then redirected by a scheduler to geographically distributed datacenters for processing.
The scheduler's decisions may depend on several mutually interacting (and in some case conflicting) objectives such
as minimizing the electricity cost, the carbon-footprint and the response time.
%, reducing transmission delays and transmission
%costs etc.
The paper \cite{Qureshi2009} is one of the first studies about GLB. In particular,
it focusses the attention on the key issues fostering the use of GLB such
as different energy markets (e.g., day-ahead and real-time markets), and temporal or geographical energy price variations.
%, and
%services supported by multiple geographical datacenters that already include
%geographical load balancing mechanisms.
The GLB represents the combination of these basic ingredients with the use of energy related metrics in the scheduler decisions.
In this manner it is possible to account for different workload conditions, and
time and geographical variability of the electricity costs.

In the last years other studies addressed the same problem by adding different scheduling constraints
and/or by optimizing different metrics (see \cite{Rao2010}, \cite{Rao2012}, \cite{Leana2012}, \cite{GuoBatterie2011},
\cite{WiermanOnline2012}, \cite{WiermanSigmetics2011}).
For instance, the papers \cite{Rao2010} and \cite{WiermanSigmetics2011} introduce additional constraints for accounting QoS guarantees;
while the interaction between GLB and smart grids, and then the exploitation of the workload demand-response capability
have been addressed in \cite{Rao2010}.
Furthermore, the interaction of energy storage systems and GLB has been addressed in \cite{GuoBatterie2011}.
Indeed, storage systems can be used to smooth the variability of power supply and this is very important when the datacenters
are powered by renewable sources.

Several studies pointed out that large datacenters are extremely expensive to maintain and this has
encouraged the development of architectures \hspace{1pt} that interconnects multiple micro-datacenters \cite{Bianchini2012}.
This trend influenced our work because workload scheduling among a large number of interconnected datacenters gives rise to
computational problems (e.g., see the summary of the techniques used in geographical load balancing in \cite{RahmanLK14}).

% ----
The works closest to ours are \cite{WiermanSigmetics2011} and \cite{WiermanOnline2012}, where geographical load balancing is driven by time-varying energy prices, that can be due to a significant local production from renewable sources. While in these papers energy prices are considered to be known in advance over some future time-horizon,  in our case renewable energy production is a stochastic process and scheduling is decided on the basis of the current state of the system.

%The approach proposed in our paper is different from that proposed in \cite{WiermanSigmetics2011} (and 
%in \cite{WiermanOnline2012}) because these works assume the knowledge of the energy prices (for a give time interval) 
%and then the schedule optimizes according a given set of objective functions. 
%On the other hand, in our approach, the energy prices are driven by stochastic processes that, in the current investigation, are simple two states on-off CTMCs but, by increasing the complexity of the analysis, these processes might account for a more complex dynamics.
 
% MICRODATACENTERS
% APPROCCI ANALITICI
% CONFRONTO CON IL NOSTRO PAPER

